Understanding the Impacts of Stellar Companions on Planet Formation and Evolution: A Survey of Stellar and Planetary Companions within 25 pc

We explore the impact of outer stellar companions on the occurrence rate of giant planets detected with radial velocities. We searched for stellar and planetary companions to a volume-limited sample of solar-type stars within 25 pc. Using adaptive optics imaging from the Lick 3m and Palomar 200" Telescopes, we characterized the multiplicity of our sample stars, down to the bottom of the main sequence. With these data, we confirm field star multiplicity statistics from previous surveys. We combined three decades of radial velocity data from the California Planet Search with new RV data from Keck/HIRES and APF/Levy to search for planets in the same systems. Using an updated catalog of both stellar and planetary companions and injection/recovery tests to determine our sensitivity, we measured the occurrence rate of planets among the single and multiple star systems. We found that planets with masses of 0.1-10 $M_{Jup}$ and semi-major axes of 0.1-10 AU have an occurrence rate of $0.18^{+0.04}_{-0.03}$ planets per single star, and $0.12\pm0.04$ planets per binary primary. Only one planet-hosting binary system in our sample had a binary separation $<100$ AU, and none had a separation $<50$ AU. We found planet occurrence rates of $0.20^{+0.07}_{-0.06}$ planets per star for binaries with separation $a_B > 100$ AU, and $0.04^{+0.04}_{-0.02}$ planets per star for binaries with separation $a_B<100$ AU. The similarity in the planet occurrence rate around single stars and wide primaries implies that wide binary systems should host more planets than single star systems, since they have more potential host stars. We estimated a system-wide planet occurrence rate of 0.3 planets per wide binary system for binaries with separations $a_B > 100$ AU. Finally, we found evidence that giant planets in binary systems have a different semi-major axis distribution than their counterparts in single star systems.

==> tables/occurrence_rates.tex <==
\hline

